Exploiting Adjoints in Property Directed Reachability Analysis

We formulate, in lattice-theoretic terms, two novel algorithms inspired by Bradley's property directed reachability algorithm. For finding safe invariants or counterexamples, the first algorithm exploits over-approximations of both forward and backward transition relations, expressed abstractly by the notion of adjoints. In the absence of adjoints, one can use the second algorithm, which exploits lower sets and their principals. As a notable example of application, we consider quantitative reachability problems for Markov Decision Processes.

==> __latexindent_temp.tex <==
\section{Implementation and Experiments}\label{sec:experiments}

We first developed, using Haskell and exploiting its abstraction features,  a common template that accommodates both {\APDR} and {\ADPDR}.
It is a  program parametrized by two lattices---used for positive chains and negative sequences, respectively---and by a heuristic.


For our experiments, we instantiated the template to \ADPDR{} for MDPs (letting $L=[0,1]^{S}$), with three different heuristics: \verb|hCoB| and \verb|hCo01| from Proposition~\ref{prop:genlegit};  and  \verb|hCoS|  introduced below. Besides the template ($\sim$100 lines),  we needed $\sim$140 lines to account for \verb|hCoB| and \verb|hCo01|, and additional $\sim$100 lines to further obtain \verb|hCoS|. All this indicates a clear benefit of our abstract theory: a general template can itself be coded succinctly;  instantiation to concrete problems is easy, too, thanks to an explicitly specified interface of heuristics.


Our implementation accepts MDPs  expressed in a symbolic format
inspired by Prism models~\cite{KwiatkowskaNP11}, in which states are variable valuations and  transitions are described by symbolic functions (they can be segmented with symbolic guards $\{\text{guard}_i\}_{i}$).
We use rational arithmetic
(\verb|Rational| in Haskell) for probabilities
to limit the impact of rounding errors.







\begin{table}[tbp]\scriptsize
  \caption{Experimental results on MC benchmarks. $|S|$ is the number of states, $P$ is the
reachability probability, $\lambda$ is the threshold in the problem $P\le_{?} \lambda$ (shaded if the answer is no). The other columns show the average execution time in seconds; TO is timeout (\SI{900}{\second}); MO is out-of-memory.
For \ADPDR{} and LT-PDR
we used the \texttt{tasty-bench} Haskell package and repeated executions until std.\ dev.\ is $<$ 5\% (at least three execs). For PrIC3 and Storm, we made five executions. Storm's execution does not depend on $\lambda$: it seems to answer to queries of the form $P\le_{?} \lambda$ by calculating $P$.
} \label{tb:mc}
\begin{lrbox}{\lstbox}\begin{minipage}{\textwidth}
  \npdecimalsign{.}
  \nprounddigits{3}
	       \begin{tabular}{ccccccccccccccc}
    	       \toprule
    	       Benchmark & $|S|$ &
    	       %
    	       $P$
    	       & $\lambda$
    	       &\multicolumn{3}{c}{\ADPDR}
    	       &%
     	       LT-PDR
    	       &\multicolumn{4}{c}{PrIC3}
    	       &\multicolumn{3}{c}{Storm}
    	       \\\cmidrule(lr){5-7} \cmidrule(lr){9-12} \cmidrule(lr){13-15}
    	       &&&&\verb|hCoB| &\verb|hCo01| &\verb|hCoS|
    	       & &none & lin. & pol. & hyb. &sp.-num. &sp.-rat. &sp.-sd. \\
    	       \midrule\midrule
    	       \multirow{4}{*}{Grid} & \multirow{2}{*}{$10^2$} & \multirow{2}{*}{0.033} & 0.3 & 0.013 &0.022 & 0.659 & 0.343 & 1.383 &23.301 &MO &MO &\multirow{2}{*}{0.010} &\multirow{2}{*}{0.010} &\multirow{2}{*}{0.010} \\
               &   &   & 0.2 & 0.013 &0.031 & 0.657 & 0.519 & 1.571 &26.668 &TO &MO \\
    	       \cmidrule[0.5pt](r){2-15}
     	       & \multirow{2}{*}{$10^3$} & \multirow{2}{*}{$<$0.001} & 0.3 & 1.156 &2.187 & 5.633 & 126.441 & TO &TO &TO &MO &\multirow{2}{*}{0.010} &\multirow{2}{*}{0.017} &\multirow{2}{*}{0.011} \\
               &   &   & 0.2 & 1.146 &2.133 & 5.632 & 161.667 & TO &TO &TO &MO \\
    	       \midrule
    	       \multirow{3}{*}{BRP} & \multirow{3}{*}{$10^3$} & \multirow{3}{*}{0.035} & 0.1 & 12.909 &7.969 & 55.788 & TO & TO &TO &MO &MO &\multirow{3}{*}{0.012} &\multirow{3}{*}{0.018} &\multirow{3}{*}{0.011} \\
               &   &   & \cellcolor{gray!25}0.01  & 1.977 &8.111 & 5.645 & 21.078 & 60.738 &626.052 &524.373 &823.082  \\
               &   &   & \cellcolor{gray!25}0.005 & 0.604 &2.261  & 2.709 & 1.429 & 12.171 &254.000 &197.940 &318.840  \\
      	       \midrule
    	       \multirow{8}{*}{\parbox{4em}{Zero- Conf}} & \multirow{4}{*}{$10^2$} & \multirow{4}{*}{0.5} & 0.9 &1.217 &68.937  & 0.196 & TO & 19.765 &136.491 &0.630 &0.468 &\multirow{4}{*}{0.010} &\multirow{4}{*}{0.018} &\multirow{4}{*}{0.011} \\
               &   &   & 0.75 & 1.223 & 68.394 & 0.636 & TO & 19.782 &132.780 &0.602 &0.467  \\
               &   &   & 0.52 & 1.228 & 60.024 & 0.739& TO & 19.852 &136.533 &0.608 &0.474  \\
               &   &   & \cellcolor{gray!25}0.45 &$<$0.001 & 0.001 & 0.001 & $<$0.001 & 0.035 &0.043 &0.043 &0.043 \\
    	       \cmidrule[0.5pt](r){2-15}
     	       & \multirow{4}{*}{$10^4$} & \multirow{4}{*}{0.5} & 0.9 &MO & TO & 7.443 & TO & TO &TO &0.602 &0.465 &\multirow{4}{*}{0.037} &\multirow{4}{*}{262.193} &\multirow{4}{*}{0.031} \\
               &   &   & 0.75 & MO & TO & 15.223 & TO & TO &TO &0.599 &0.470  \\
               &   &   & 0.52 & MO & TO & TO & TO &TO &TO &0.488 & 0.475 \\
               &   &   & \cellcolor{gray!25}0.45 &0.108 & 0.119 & 0.169 & 0.016 & 0.035 &0.040 &0.040 &0.040  \\
    	       \midrule
    	       \multirow{4}{*}{Chain} & \multirow{4}{*}{$10^3$} & \multirow{4}{*}{0.394} & 0.9 & 36.083 & TO & 0.478 & TO & 269.801 &TO &0.938 &0.686 &\multirow{4}{*}{0.010} &\multirow{4}{*}{0.014} &\multirow{4}{*}{0.011} \\
               &   &   & 0.4 & 35.961 & TO & 394.955 & TO & 271.885 &TO &0.920 &TO\\
               &   &   & \cellcolor{gray!25}0.35 & 101.351 & TO & 454.892 & 435.199 & 238.613 &TO &TO &TO  \\
               &   &   & \cellcolor{gray!25}0.3 & 62.036 & 463.981 & 120.557 & 209.346 & 124.829 &746.595 &TO &TO \\
    	       \midrule
    	       \multirow{4}{*}{\parbox{4em}{Double- Chain}} & \multirow{4}{*}{$10^3$} & \multirow{4}{*}{0.215} & 0.9 & 12.122 & 7.318 & TO & TO & TO &TO &1.878 &2.053 &\multirow{4}{*}{0.011} &\multirow{4}{*}{0.018} &\multirow{4}{*}{0.010} \\
               &   &   & 0.3 & 12.120 & 20.424 & TO & TO & TO &TO &1.953 &2.058 \\
               &   &   & 0.216 & 12.096 & 19.540 & TO & TO & TO &TO &172.170 &TO \\
               &   &   & \cellcolor{gray!25}0.15 & 12.344 & 16.172 & TO & 16.963 & TO &TO &TO &TO \\
    	       \midrule
    	       \multirow{4}{*}{\parbox{4em}{Haddad- Monmege}} & \multirow{2}{*}{$41$} & \multirow{2}{*}{0.7} & 0.9 & 0.004 & 0.009 &8.528 & TO & 1.188 &31.915 &TO &MO &\multirow{2}{*}{0.011} &\multirow{2}{*}{0.011} &\multirow{2}{*}{1.560} \\
               &   &   & 0.75 & 0.004 & 0.011 & 2.357 & TO & 1.209 &32.143 &TO &712.086 \\
    	       \cmidrule[0.5pt](r){2-15}
     	       & \multirow{2}{*}{$10^3$} & \multirow{2}{*}{0.7} & 0.9 & 59.721 & 61.777 &TO & TO & TO &TO &TO &TO &\multirow{2}{*}{0.013} &\multirow{2}{*}{0.043} &\multirow{2}{*}{TO} \\
               &   &   & 0.75 & 60.413 & 63.050 & TO & TO & TO &TO &TO &TO \\
    	       \bottomrule
  	       \end{tabular}
\end{minipage}\end{lrbox}
\scalebox{.84}{\centering\usebox\lstbox}
\end{table}

\myparagraph{Heuristics.}
The three heuristics (\verb|hCoB|, \verb|hCo01|, \verb|hCoS|) use the same choices in (Candidate) and (Decide),
as defined in \eqref{eq:secondterminatingheuristics},
but different ones in (Conflict).

The third heuristics \verb|hCoS| is a \emph{symbolic} variant of
\verb|hCoB|; it relies on our symbolic model format.
It uses $z_{S}$ for $z$ in (Conflict), where $z_{S}(s)=z_{B}(s)$ if $r_{s}\neq 0$ or $\mathcal{Z}_k=\emptyset$. The definition of $z_{S}(s)$ otherwise is notable: we use a piecewise affine function $(t_{i}\cdot s + u_{i})_{i}$ for $z_{S}(s)$,
where the affine functions $(t_{i}\cdot s + u_{i})_{i}$ are guarded by the same guards $\{\text{guard}_i\}_{i}$ of the MDP's transition function. We let the SMT solver Z3~\cite{MouraB08} search for the values of the coefficients $t_{i}, u_{i}$, so that $z_{S}$ satisfies the requirements of (Conflict) (namely $b(x_{k-1})(s) \leq z_{S}(s) \leq 1$ for each $s\in S$ with $r_s=0$), together with the condition
 $b (z_{S}) \leq z_{S}$ for faster convergence.
If the search is unsuccessful, we give up
\verb|hCoS| and fall back on the heuristic \verb|hCoB|.



As a task common to the three heuristics, we need to calculate $\mathcal{Z}_k = \{d \in \mathcal{G}_k \mid b(x_{k-1}) \leq d\}$ in (Conflict) (see~(\ref{eq:heuristicsZConflict})). Rather than computing the whole set $\mathcal{G}_k$ of generating points of the linear inequality that defines $Y_{k}$, we implemented an ad-hoc algorithm that crucially exploits the condition $b(x_{k-1}) \leq d$ for pruning.





\myparagraph{Experiment Settings.}
We conduct the experiments on Ubuntu 18.04 and AWS t2.xlarge (4 CPUs, 16 GB memory, up to 3.0 GHz Intel Scalable Processor). We used several Markov chain (MC)
 benchmarks
and a couple of MDP ones.


\myparagraph{Research Questions.} We wish to address the following questions.
\begin{description}
 \item[RQ1] Does \ADPDR{} advance the state-of-the-art performance of \emph{PDR} algorithms for probabilistic model checking?
 \item[RQ2] How does \ADPDR{}'s performance compare against \emph{non-PDR} algorithms for probabilistic model checking?
 \item[RQ3] Does the  theoretical framework of \ADPDR{} successfully guide the discovery of various heuristics with practical performance?
 \item[RQ4] Does \ADPDR{} successfully manage nondeterminism in MDPs
  (that is absent in MCs)?
\end{description}

\myparagraph{Experiments on
MCs (Table~\ref{tb:mc}).}
We used six
benchmarks:  Haddad\hyp{}Monmege  is from~\cite{HartmannsKPQR19}; the others are from~\cite{BatzJKKMS20,KoriCAV22}.
We compare
  \ADPDR (with three heuristics) against LT-PDR~\cite{KoriCAV22}, PrIC3 (with four  heuristics \emph{none}, \emph{lin.}, \emph{pol.}, \emph{hyb.}, see~\cite{BatzJKKMS20}), and Storm 1.5~\cite{DehnertJK017}.
Storm is a recent comprehensive toolsuite that implements different algorithms and solvers. Among them, our comparison is against \kori{\emph{sparse-numeric}, \emph{sparse-rational}, and \emph{sparse-sound}}. The \emph{sparse} engine uses explicit state space representation by sparse matrices; this is unlike another representative \emph{dd} engine that uses symbolic BDDs. (We did not use \emph{dd} since it often reported errors, and was overall slower than \emph{sparse}.)
 \emph{Sparse-numeric}  is a value-iteration (VI) algorithm;  \emph{sparse-rational}  solves linear (in)equations using rational arithmetic;
 \kori{\emph{sparse-sound} is a sound VI algorithm~\cite{QuatmannK18}}.


\begin{table}[tbp]
  \scriptsize
  \caption{Experimental results on MDP benchmarks. The legend is the same as Table~\ref{tb:mc}, except that $P$ is now the maximum reachability probability.} \label{tb:mdp}
\begin{lrbox}{\lstbox}\begin{minipage}{\textwidth}
\centering
\begin{tabular}{cccccccccc}
    \toprule
    Benchmark & $|S|$ &
    $P$\
    & $\lambda$
    &\multicolumn{3}{c}{\ADPDR}
    &\multicolumn{3}{c}{Storm}
    \\\cmidrule(lr){5-7}\cmidrule{8-10}
    &&&&\verb|hCoB| &\verb|hCo01| &\verb|hCoS| &sp.-num &sp.-rat. &sp.-sd. \\
    \midrule\midrule
    \multirow{3}{*}{CDrive2} &\multirow{3}{*}{38} &\multirow{3}{*}{0.865} &0.9 &MO &0.172 &TO &\multirow{3}{*}{0.019} &\multirow{3}{*}{0.019} &\multirow{3}{*}{0.018}\\
    &&&\cellcolor{gray!25}0.75 &MO &0.058 &TO\\
    &&&\cellcolor{gray!25}0.5 &0.015 &0.029 &86.798 \\
    \midrule
    \multirow{3}{*}{TireWorld} &\multirow{3}{*}{8670} &\multirow{3}{*}{0.233} &0.9 &MO &3.346 &TO  &\multirow{4}{*}{0.070}&\multirow{4}{*}{0.164} &\multirow{4}{*}{0.069}\\
    &&&0.75 &MO &3.337 &TO \\
    &&&0.5 &MO &6.928 &TO \\
    &&&\cellcolor{gray!25}0.2 &4.246 &24.538 &TO \\
    \bottomrule
\end{tabular}
\end{minipage}\end{lrbox}
\scalebox{.85}{\centering\usebox\lstbox}
\end{table}




\myparagraph{Experiments on MDPs (Table~\ref{tb:mdp}).}
We used two benchmarks  from~\cite{HartmannsKPQR19}. We compare \ADPDR only against Storm, since RQ1 is already addressed using MCs (besides, PrIC3 did not run for MDPs).






\myparagraph{Discussion.} The experimental results suggest the following answers to the RQs.

\textbf{RQ1}. The performance advantage of \ADPDR{}, over both LT-PDR and PrIC3, was clearly observed throughout the benchmarks.
\ADPDR{} outperformed LT-PDR, thus confirming empirically the theoretical observation in Section~\ref{ssec:LTPDRvsADPDR}. The profit is particularly evident in those instances whose answer is positive.
\ADPDR{} generally outperformed PrIC3, too.
Exceptions are in ZeroConf, Chain and DoubleChain, where PrIC3 with  polynomial (pol.) and hybrid (hyb.) heuristics performs well. This seems to be thanks to the expressivity of the polynomial template in PrIC3, which is a possible enhancement we are yet to implement (currently our symbolic heuristic \verb|hCoS| uses only the affine template).

\textbf{RQ2}. The comparison with Storm is interesting.  Note first that Storm's \emph{sparse-numeric} algorithm is a VI algorithm that gives a guaranteed lower bound \emph{without guaranteed convergence}. Therefore  its positive answer to $P\le_{?}\lambda$ may not be correct. Indeed, for Haddad-Monmege with $|S|\sim 10^{3}$, it answered $P=0.5$ which is wrong. This is in contrast with PDR algorithms that discovers an explicit witness for  $P\le\lambda$ via their positive chain.

Storm's \emph{sparse-rational} algorithm is precise.
It was faster than PDR algorithms in many benchmarks, although \ADPDR was better or comparable in ZeroConf ($10^4$) and Haddad-Monmege ($41$), for $\lambda$ such that $P\le\lambda$ is true. We believe this suggests a general advantage of PDR algorithms, namely to accelerate the search for an invariant-like witness for safety.

\kori{Storm's \emph{sparse-sound} algorithm is a sound VI algorithm that returns correct answers aside numerical errors.
The results were similar to those of sparse-numeric, except for two benchmarks of Haddad-Monmege: sparse-sound returned correct answers but was much slower than sparse-numeric.
For both benchmarks, \ADPDR{} outperformed sparse-sound.  This suggests that there are several cases where \ADPDR{} performs better than sound VI algorithms.}

It seems that a big part of Storm's good performance is attributed to the sparsity of state representation. This is notable in the comparison of the two instances of Haddad-Monmege ($41$ vs.\ $10^3$): while Storm handles both of them easily, \ADPDR{} struggles a bit in the bigger instance. Our implementation can be extended to use sparse representation, too; this is future work.


\textbf{RQ3}. We derived the three heuristics (\verb|hCoB|, \verb|hCo01|, \verb|hCoS|) exploiting the theory of \ADPDR{}. The experiments show that each heuristic has its own strength. For example, \verb|hCo01| is slower than \verb|hCoB| for MCs, but it is much better for MDPs. In general, there is no silver bullet heuristic, so coming up with a variety of them is important. The experiments suggest that our theory of \ADPDR{} provides great help in doing so.


\textbf{RQ4}. Table~\ref{tb:mdp}  shows that \ADPDR{} can handle nondeterminism well: once a suitable heuristic is chosen, its performances on MDPs and on MCs of similar size are comparable.
It is also interesting that better-performing heuristics vary, as we discussed above.


\myparagraph{Conclusion.}
\ADPDR{} clearly outperforms  existing probabilistic PDR algorithms in many benchmarks. It also compares well with Storm---a highly sophisticated toolsuite---in a couple of benchmarks. These are notable especially given that \ADPDR{} currently lacks enhancing features such as richer symbolic templates and sparse representation (adding which is future work). Overall, we believe that \ADPDR{} \emph{confirms the potential of PDR algorithms in probabilistic model checking}. Through the three heuristics, we also observed the value of an abstract general theory in devising heuristics in PDR, which is probably true of verification algorithms in general besides PDR.






==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_EXCMD	mixed	/number, pattern, mixed, or combineV2/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROC_CWD	/Users/kotapiku/ghq/github.com/kotapiku/PDR-pisa/CAV2023-final_arXiv/	//
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	5.9.0	/3a88dc2/
Adjoint PDR	30-APDR.tex	/^\\section{Adjoint PDR}\\label{sec:APDR}$/;"	r
D	00-macros.tex	/^\\newcommand{\\D}{\\mathcal{D}}$/;"	r
Heuristics	30-APDR.tex	/^\\subsection{Heuristics}\\label{sec:heuristics}$/;"	r
Htrz	00-macros.tex	/^\\newcommand{\\Htrz}[3]{{\\stackrel{#1}{\\to}}_{#2}^{#3}}$/;"	r
Implementation and Experiments	80-experiments.tex	/^\\section{Implementation and Experiments}\\label{sec:experiments}$/;"	r
Implementation and Experiments	__latexindent_temp.tex	/^\\section{Implementation and Experiments}\\label{sec:experiments}$/;"	r
Instantiating {\\ADPDR	70-probabilistic.tex	/^\\section{Instantiating {\\ADPDR} for MDPs}\\label{sec:MDP}$/;"	r
Introduction	10-intro.tex	/^\\section{Introduction}\\label{sec:intro}$/;"	r
KTomega	00-macros.tex	/^\\newcommand{\\KTomega}{$\\text{KT}^{\\omega}$}$/;"	r
KTseq	00-macros.tex	/^\\newcommand{\\KTseq}{KT$_\\text{adj}$ sequence}$/;"	r
KTstar	00-macros.tex	/^\\newcommand{\\KTstar}{$\\text{KT}^{\\*}$}$/;"	r
Kleeneseq	00-macros.tex	/^\\newcommand{\\Kleeneseq}{Kleene$_\\text{adj}$ sequence}$/;"	r
Nat	00-macros.tex	/^\\newcommand{\\Nat}{\\mathbb{N}}$/;"	r
Negative Termination	40-termination.tex	/^\\subsection{Negative Termination}\\label{sec:termination}$/;"	r
Pf	00-macros.tex	/^\\newcommand{\\Pf}{\\mathcal{P}}$/;"	r
Preliminaries and Notation	20-background.tex	/^\\section{Preliminaries and Notation}\\label{sec:preliminaries}$/;"	r
Progression	30-APDR.tex	/^\\subsection{Progression}\\label{sec:progression}$/;"	r
Recovering Adjoints with Lower Sets	60-downset.tex	/^\\section{Recovering Adjoints with Lower Sets}\\label{sec:downset}$/;"	r
Set	00-macros.tex	/^\\newcommand{\\Set}{\\mathbf{Set}}$/;"	r
abstract	cav2023.tex	/^\\begin{abstract}$/;"	r
align	30-APDR.tex	/^\\begin{align}$/;"	r
align*	20-background.tex	/^\\begin{align*}%$/;"	r
align*	30-APDR.tex	/^{\\footnotesize \\begin{align*}$/;"	r
align*	70-probabilistic.tex	/^ {\\footnotesize \\begin{align*}$/;"	r
align*	70-probabilistic.tex	/^\\begin{align*}$/;"	r
array	20-background.tex	/^\\begin{array}{c}$/;"	r
array	30-APDR.tex	/^\\begin{array}{r|ll}$/;"	r
array	70-probabilistic.tex	/^\\[\\begin{array}{rc|c|c}$/;"	r
auxproof	10-intro.tex	/^\\begin{auxproof}$/;"	r
bmatrix	00-macros.tex	/^\\newcommand{\\cvec}[4]{\\!{\\tiny{ \\!\\begin{bmatrix} #1 \\\\ #2 \\\\ #3 \\\\#4 \\end{bmatrix}/;"	r
bmatrix	70-probabilistic.tex	/^\\[ p^\\downarrow = \\{\\,\\cvec{v_0}{v_1}{v_2}{v_3} \\mid {\\tiny{ \\!\\begin{bmatrix} 1 & 0 & /;"	r
bmatrix	70-probabilistic.tex	/^\\\\ 2&2&2&0 \\\\ \\frac{10}{3}&0&\\frac{8}{3}&0 \\end{bmatrix}\\!}} \\cdot \\cvec{v_0}{v_1}{v_2/;"	r
bmatrix	70-probabilistic.tex	/^\\mathcal{F}^0 & \\defeq &  \\{\\,\\cvec{v_0}{v_1}{v_2}{v_3} \\mid {\\tiny{ \\!\\begin{bmatrix} /;"	r
bmatrix	70-probabilistic.tex	/^\\mathcal{F}^1 & \\defeq &   \\{\\,\\cvec{v_0}{v_1}{v_2}{v_3} \\mid {\\tiny{ \\!\\begin{bmatrix}/;"	r
bmatrix	70-probabilistic.tex	/^\\mathcal{F}^2 & \\defeq & \\{\\,\\cvec{v_0}{v_1}{v_2}{v_3} \\mid {\\tiny{ \\!\\begin{bmatrix} 3/;"	r
bmatrix	70-probabilistic.tex	/^\\mathcal{F}^3 & \\defeq & \\{\\,\\cvec{v_0}{v_1}{v_2}{v_3} \\mid {\\tiny{ \\!\\begin{bmatrix} 0/;"	r
bmatrix	70-probabilistic.tex	/^\\mathcal{F}^4 & \\defeq & \\{\\,\\cvec{v_0}{v_1}{v_2}{v_3} \\mid  {\\tiny{ \\!\\begin{bmatrix} /;"	r
cases	70-probabilistic.tex	/^      b_{\\alpha}(d)(s) \\defeq \\begin{cases}$/;"	r
cases	70-probabilistic.tex	/^      p(s)\\defeq  \\begin{cases}$/;"	r
cases	70-probabilistic.tex	/^ b(d)(s) \\defeq  \\begin{cases}$/;"	r
cases*	30-APDR.tex	/^\\begin{cases*}$/;"	r
cases*	70-probabilistic.tex	/^\\begin{cases*}$/;"	r
codeNT	30-APDR.tex	/^\\begin{codeNT}$/;"	r
codeNT	60-downset.tex	/^\\begin{codeNT}$/;"	r
conf	00-macros.tex	/^\\newcommand{\\conf}[1]{}$/;"	r
cor:ADPDRtermination	70-probabilistic.tex	/^\\begin{corollary}\\label{cor:ADPDRtermination}$/;"	r
cor:negativetermiantion	40-termination.tex	/^\\begin{corollary}\\label{cor:negativetermiantion}$/;"	r
corollary	40-termination.tex	/^\\begin{corollary}\\label{cor:negativetermiantion}$/;"	r
corollary	70-probabilistic.tex	/^\\begin{corollary}\\label{cor:ADPDRtermination}$/;"	r
cvec	00-macros.tex	/^\\newcommand{\\cvec}[4]{\\!{\\tiny{ \\!\\begin{bmatrix} #1 \\\\ #2 \\\\ #3 \\\\#4 \\end{bmatrix}/;"	r
def:neg_seq	30-APDR.tex	/^\\begin{definition}[negative sequence] \\label{def:neg_seq}$/;"	r
def:posi_seq	30-APDR.tex	/^  \\begin{definition}[positive chain] \\label{def:posi_seq}$/;"	r
definition	30-APDR.tex	/^  \\begin{definition}[positive chain] \\label{def:posi_seq}$/;"	r
definition	30-APDR.tex	/^\\begin{definition}[legit heuristic]$/;"	r
definition	30-APDR.tex	/^\\begin{definition}[negative sequence] \\label{def:neg_seq}$/;"	r
definition	60-downset.tex	/^\\begin{definition}[Kleene sequence, from~\\cite{KoriCAV22}]$/;"	r
description	80-experiments.tex	/^\\begin{description}$/;"	r
description	__latexindent_temp.tex	/^\\begin{description}$/;"	r
displaymath	20-background.tex	/^\\begin{displaymath}$/;"	r
displaymath	70-probabilistic.tex	/^  \\begin{displaymath}$/;"	r
document	cav2023.tex	/^\\begin{document}$/;"	r
draft	10-intro.tex	/^\\subsection*{draft}$/;"	r
eg:simple	20-background.tex	/^\\begin{example}[Safety problem for transition systems] \\label{eg:simple}$/;"	r
enumerate	30-APDR.tex	/^\\begin{enumerate}%$/;"	r
enumerate	30-APDR.tex	/^\\begin{enumerate}\\setcounter{enumi}{0}$/;"	r
enumerate	30-APDR.tex	/^\\begin{enumerate}\\setcounter{enumi}{2}$/;"	r
eq:EMlaw	60-downset.tex	/^\\begin{equation}\\label{eq:EMlaw}$/;"	r
eq:Ix1	30-APDR.tex	/^ i \\sqsubseteq x_1  \\tag{P1} \\label{eq:Ix1}\\\\$/;"	r
eq:KNfpthm	20-background.tex	/^\\begin{equation*}\\label{eq:KNfpthm}$/;"	r
eq:Kleenefpthm	20-background.tex	/^\\label{eq:Kleenefpthm}$/;"	r
eq:Pepsilon	30-APDR.tex	/^\\text{If }\\vec{y}\\neq \\varepsilon\\text{ then }p \\sqsubseteq y_{n-1}  \\tag{N1}\\label{eq:P/;"	r
eq:chainsadjoint	20-background.tex	/^\\begin{equation}\\label{eq:chainsadjoint}$/;"	r
eq:coinductionproofprinciple	20-background.tex	/^\\begin{equation}\\label{eq:coinductionproofprinciple}$/;"	r
eq:heuristicsZConflict	70-probabilistic.tex	/^\\begin{equation}\\label{eq:heuristicsZConflict}$/;"	r
eq:iff	20-background.tex	/^\\begin{equation}\\label{eq:iff}$/;"	r
eq:invi	30-APDR.tex	/^1\\leq k \\leq n \\tag{I1} \\label{eq:invi} \\\\$/;"	r
eq:kleeneadjoint	20-background.tex	/^\\begin{equation}\\label{eq:kleeneadjoint}$/;"	r
eq:lowersetadjunction	60-downset.tex	/^  \\begin{equation}\\label{eq:lowersetadjunction}$/;"	r
eq:negativeG	30-APDR.tex	/^\\forall j\\in[k,n-2]\\text{, }g(y_{j+1}) \\sqsubseteq y_j  \\tag{N2}\\label{eq:negativeG}$/;"	r
eq:positiveF	30-APDR.tex	/^\\forall j\\in[0, n-2]\\text{, }f(x_j) \\sqsubseteq x_{j+1} \\tag{P3}\\label{eq:positiveF} \\\\$/;"	r
eq:positiveG	30-APDR.tex	/^\\forall j\\in[0, n-2]\\text{, }x_j \\sqsubseteq g(x_{j+1}) \\tag{P3a} \\label{eq:positiveG}$/;"	r
eq:positivechain	30-APDR.tex	/^\\forall j\\in[0, n-2]\\text{, }x_j \\sqsubseteq x_{j+1} \\tag{I2}\\label{eq:positivechain}$/;"	r
eq:positiveinitialfinal	30-APDR.tex	/^\\forall j \\in [0, n-1] \\text{, } (f \\sqcup i)^j (\\bot) \\sqsubseteq x_j \\sqsubseteq (g \\s/;"	r
eq:positivenegative	30-APDR.tex	/^\\forall j \\in [k, n - 1] \\text{, } x_j \\not\\sqsubseteq y_j \\tag{PN} \\label{eq:positiveneg/;"	r
eq:secondterminatingheuristics	70-probabilistic.tex	/^\\begin{equation}\\label{eq:secondterminatingheuristics}$/;"	r
eq:simple	30-APDR.tex	/^\\begin{equation}\\label{eq:simple}$/;"	r
eq:x0bot	30-APDR.tex	/^\\quad x_0 = \\bot \\tag{I0}\\label{eq:x0bot} \\\\$/;"	r
eq:xP	30-APDR.tex	/^ x_{n-2} \\sqsubseteq p  \\tag{P2}\\label{eq:xP}\\\\$/;"	r
equation	20-background.tex	/^\\begin{equation}\\label{eq:chainsadjoint}$/;"	r
equation	20-background.tex	/^\\begin{equation}\\label{eq:coinductionproofprinciple}$/;"	r
equation	20-background.tex	/^\\begin{equation}\\label{eq:iff}$/;"	r
equation	20-background.tex	/^\\begin{equation}\\label{eq:kleeneadjoint}$/;"	r
equation	30-APDR.tex	/^\\begin{equation}\\label{eq:simple}$/;"	r
equation	60-downset.tex	/^  \\begin{equation}\\label{eq:lowersetadjunction}$/;"	r
equation	60-downset.tex	/^\\begin{equation}\\label{eq:EMlaw}$/;"	r
equation	70-probabilistic.tex	/^\\begin{equation}\\label{eq:heuristicsZConflict}$/;"	r
equation	70-probabilistic.tex	/^\\begin{equation}\\label{eq:secondterminatingheuristics}$/;"	r
equation*	20-background.tex	/^\\begin{equation*}\\label{eq:KNfpthm}$/;"	r
ex:MDPpositive	70-probabilistic.tex	/^  \\begin{example}\\label{ex:MDPpositive}$/;"	r
ex:shortheuristicforDecide	70-probabilistic.tex	/^\\begin{example}\\label{ex:shortheuristicforDecide}$/;"	r
ex:simple-ts	30-APDR.tex	/^\\begin{example}\\label{ex:simple-ts}$/;"	r
example	20-background.tex	/^\\begin{example}[Safety problem for transition systems] \\label{eg:simple}$/;"	r
example	30-APDR.tex	/^\\begin{example}$/;"	r
example	30-APDR.tex	/^\\begin{example}\\label{ex:simple-ts}$/;"	r
example	70-probabilistic.tex	/^  \\begin{example}\\label{ex:MDPpositive}$/;"	r
example	70-probabilistic.tex	/^\\begin{example}\\label{ex:shortheuristicforDecide}$/;"	r
fig:LTS	20-background.tex	/^\\caption{The transition system of Example~\\ref{eg:simple}, with $S = \\{ s_0, \\dots s_6 \\}$ /;"	r
fig:downclosed	60-downset.tex	/^\\label{fig:downclosed}$/;"	r
fig:exDecideheuristics	70-probabilistic.tex	/^}\\label{fig:exDecideheuristics}$/;"	r
fig:invariants	30-APDR.tex	/^\\label{fig:invariants}$/;"	r
fig:naive	30-APDR.tex	/^\\caption{{\\APDR} algorithm checking $\\mu (f \\sqcup i) \\sqsubseteq p$.}\\label{fig:naive}$/;"	r
figure	20-background.tex	/^\\begin{figure}[t]$/;"	r
figure	30-APDR.tex	/^\\begin{figure}[t]$/;"	r
figure	60-downset.tex	/^\\begin{figure}[t]$/;"	r
figure	70-probabilistic.tex	/^\\begin{figure}[t]$/;"	r
itemize	10-intro.tex	/^\\begin{itemize}$/;"	r
lloop	00-macros.tex	/^\\newcommand{\\lloop}[2][-]{\\save \\POS!L(.7) \\ar@(lu,ld)_#1{#2} \\restore}$/;"	r
lrbox	30-APDR.tex	/^\\begin{lrbox}{\\lstbox}\\begin{minipage}{\\textwidth}$/;"	r
lrbox	60-downset.tex	/^\\begin{lrbox}{\\lstbox}\\begin{minipage}{\\textwidth}$/;"	r
lrbox	70-probabilistic.tex	/^\\begin{lrbox}{\\lstbox}\\begin{minipage}{\\textwidth}$/;"	r
lrbox	80-experiments.tex	/^\\begin{lrbox}{\\lstbox}\\begin{minipage}{\\textwidth}$/;"	r
lrbox	__latexindent_temp.tex	/^\\begin{lrbox}{\\lstbox}\\begin{minipage}{\\textwidth}$/;"	r
ltpdradj	00-macros.tex	/^\\newcommand{\\ltpdradj}{LT-PDR$_\\text{adj}$}$/;"	r
math	10-intro.tex	/^   \\begin{math}$/;"	r
math	10-intro.tex	/^  \\begin{math}$/;"	r
minipage	00-macros.tex	/^\\newenvironment{thmblock}{\\noindent\\begin{minipage}{\\textwidth}}{\\end{minipage}}$/;"	r
minipage	10-intro.tex	/^\\begin{minipage}{.16\\textwidth}$/;"	r
minipage	10-intro.tex	/^\\begin{minipage}{.35\\textwidth}$/;"	r
minipage	30-APDR.tex	/^\\begin{minipage}{.4\\linewidth}$/;"	r
minipage	30-APDR.tex	/^\\begin{minipage}{.5\\linewidth}$/;"	r
minipage	30-APDR.tex	/^\\begin{minipage}{.6\\linewidth}$/;"	r
minipage	30-APDR.tex	/^\\noindent \\begin{minipage}{.5\\linewidth}$/;"	r
myparagraph	00-macros.tex	/^\\newcommand{\\myparagraph}[1]{\\vspace*{.3em}\\noindent\\textbf{#1}\\;}$/;"	r
negation	00-macros.tex	/^\\newcommand{\\negation}[1]{\\vec{neg(#1)}}$/;"	r
negativefinal	30-APDR.tex	/^\\forall j\\in[k,n-1]\\text{, }g^{n-1-j}(p) \\sqsubseteq y_j \\tag{A3} \\label{negativefinal}$/;"	r
op	00-macros.tex	/^\\newcommand{\\op}{\\mathrm{op}}$/;"	r
positivefinal	30-APDR.tex	/^\\forall j \\in [1, n-1] \\text{, } x_{j-1} \\sqsubseteq g^{n-1-j}(p) \\tag{A2} \\label{positive/;"	r
prop:CanonicalChoice	30-APDR.tex	/^\\begin{proposition}[Canonical choices]\\label{prop:CanonicalChoice}$/;"	r
prop:LTPDRfinal	60-downset.tex	/^\\begin{proposition}\\label{prop:LTPDRfinal}$/;"	r
prop:genlegit	70-probabilistic.tex	/^\\begin{proposition}\\label{prop:genlegit}$/;"	r
prop:multipleLTPDR	60-downset.tex	/^\\begin{proposition}\\label{prop:multipleLTPDR}$/;"	r
prop:negativesequencefinalchain	30-APDR.tex	/^\\begin{proposition}\\label{prop:negativesequencefinalchain}$/;"	r
prop:prob_down_up	60-downset.tex	/^\\begin{proposition} \\label{prop:prob_down_up}$/;"	r
prop:progres	30-APDR.tex	/^\\begin{proposition}[Impossibility of loops]\\label{prop:progres}$/;"	r
proposition	30-APDR.tex	/^\\begin{proposition}[Canonical choices]\\label{prop:CanonicalChoice}$/;"	r
proposition	30-APDR.tex	/^\\begin{proposition}[Impossibility of loops]\\label{prop:progres}$/;"	r
proposition	30-APDR.tex	/^\\begin{proposition}\\label{prop:negativesequencefinalchain}$/;"	r
proposition	60-downset.tex	/^\\begin{proposition} \\label{prop:prob_down_up}$/;"	r
proposition	60-downset.tex	/^\\begin{proposition}\\label{prop:LTPDRfinal}$/;"	r
proposition	60-downset.tex	/^\\begin{proposition}\\label{prop:multipleLTPDR}$/;"	r
proposition	70-probabilistic.tex	/^\\begin{proposition}\\label{prop:genlegit}$/;"	r
reachablestates	00-macros.tex	/^\\newcommand{\\reachablestates}{\\mathcal{S}^r}$/;"	r
rloop	00-macros.tex	/^\\newcommand{\\rloop}[2][-]{\\save \\POS!R(.7) \\ar@(ru,rd)^#1{#2} \\restore}$/;"	r
sec:APDR	30-APDR.tex	/^\\section{Adjoint PDR}\\label{sec:APDR}$/;"	r
sec:MDP	70-probabilistic.tex	/^\\section{Instantiating {\\ADPDR} for MDPs}\\label{sec:MDP}$/;"	r
sec:downset	60-downset.tex	/^\\section{Recovering Adjoints with Lower Sets}\\label{sec:downset}$/;"	r
sec:experiments	80-experiments.tex	/^\\section{Implementation and Experiments}\\label{sec:experiments}$/;"	r
sec:experiments	__latexindent_temp.tex	/^\\section{Implementation and Experiments}\\label{sec:experiments}$/;"	r
sec:heuristics	30-APDR.tex	/^\\subsection{Heuristics}\\label{sec:heuristics}$/;"	r
sec:intro	10-intro.tex	/^\\section{Introduction}\\label{sec:intro}$/;"	r
sec:preliminaries	20-background.tex	/^\\section{Preliminaries and Notation}\\label{sec:preliminaries}$/;"	r
sec:progression	30-APDR.tex	/^\\subsection{Progression}\\label{sec:progression}$/;"	r
sec:termination	40-termination.tex	/^\\subsection{Negative Termination}\\label{sec:termination}$/;"	r
ssec:ADPDR	60-downset.tex	/^\\subsection{{\\ADPDR}: Positive Chain in $L$, Negative Sequence in $L^\\downarrow$}\\label{ssec/;"	r
ssec:LTPDRvsADPDR	60-downset.tex	/^\\subsection{{\\ADPDR} simulates LT-PDR}\\label{ssec:LTPDRvsADPDR}$/;"	r
states	00-macros.tex	/^\\newcommand{\\states}{\\mathcal{S}}$/;"	r
table	80-experiments.tex	/^\\begin{table}[tb]$/;"	r
table	80-experiments.tex	/^\\begin{table}[tb]\\scriptsize$/;"	r
table	__latexindent_temp.tex	/^\\begin{table}[tbp]$/;"	r
table	__latexindent_temp.tex	/^\\begin{table}[tbp]\\scriptsize$/;"	r
tabular	80-experiments.tex	/^	       \\begin{tabular}{ccccccccccccccc}$/;"	r
tabular	80-experiments.tex	/^\\begin{tabular}{cccccccccc}$/;"	r
tabular	__latexindent_temp.tex	/^	       \\begin{tabular}{ccccccccccccccc}$/;"	r
tabular	__latexindent_temp.tex	/^\\begin{tabular}{cccccccccc}$/;"	r
tb:mc	80-experiments.tex	/^} \\label{tb:mc}$/;"	r
tb:mc	__latexindent_temp.tex	/^} \\label{tb:mc}$/;"	r
tb:mdp	80-experiments.tex	/^  \\caption{Experimental results on MDP benchmarks. The legend is the same as Table~\\ref{tb:mc}/;"	r
tb:mdp	__latexindent_temp.tex	/^  \\caption{Experimental results on MDP benchmarks. The legend is the same as Table~\\ref{tb:mc}/;"	r
th:ADPDR	60-downset.tex	/^\\begin{theorem}\\label{th:ADPDR}$/;"	r
th:LT-PDR-instance-ADPDR	60-downset.tex	/^\\label{th:LT-PDR-instance-ADPDR}$/;"	r
th:soundness	30-APDR.tex	/^\\begin{theorem}[Soundness]\\label{th:soundness}$/;"	r
theorem	30-APDR.tex	/^\\begin{theorem}[Soundness]\\label{th:soundness}$/;"	r
theorem	40-termination.tex	/^\\begin{theorem}[Negative termination]\\label{thm:negativetermination}$/;"	r
theorem	60-downset.tex	/^\\begin{theorem}%$/;"	r
theorem	60-downset.tex	/^\\begin{theorem}\\label{th:ADPDR}$/;"	r
thm:negativetermination	40-termination.tex	/^\\begin{theorem}[Negative termination]\\label{thm:negativetermination}$/;"	r
todoil	00-macros.tex	/^\\newcommand{\\todoil}[1]{\\todo[inline,caption={}]{#1}}$/;"	r
todoil	00-macros.tex	/^\\newcommand{\\todoil}[1]{}$/;"	r
tr	00-macros.tex	/^\\newcommand{\\tr}[1]{\\stackrel{#1}{\\to}}$/;"	r
trz	00-macros.tex	/^\\newcommand{\\trz}[2]{{\\stackrel{#1}{\\to}}_{#2}}$/;"	r
ttp	00-macros.tex	/^\\newcommand{\\ttp}[1]{\\stackrel{#1}{\\to^+}}$/;"	r
ttr	00-macros.tex	/^\\newcommand{\\ttr}[1]{\\stackrel{#1}{\\to^*}}$/;"	r
uloop	00-macros.tex	/^\\newcommand{\\uloop}[2][-]{\\save \\POS!U(.7) \\ar@(lu,ru)^(.8){#2} \\restore}$/;"	r
wrapfigure	10-intro.tex	/^\\begin{wrapfigure}[3]{r}{0pt}$/;"	r
wrapfigure	10-intro.tex	/^\\begin{wrapfigure}[4]{r}{0pt}$/;"	r
{\\ADPDR	60-downset.tex	/^\\subsection{{\\ADPDR} simulates LT-PDR}\\label{ssec:LTPDRvsADPDR}$/;"	r
{\\ADPDR	60-downset.tex	/^\\subsection{{\\ADPDR}: Positive Chain in $L$, Negative Sequence in $L^\\downarrow$}\\label{ssec/;"	r

